AFCL: Analytic Federated Continual Learning for Spatio-Temporal Invariance of Non-IID Data

Federated Continual Learning (FCL) enables distributed clients to collaboratively train a global model from online task streams in dynamic real-world scenarios. However, existing FCL methods face challenges of both spatial data heterogeneity among distributed clients and temporal data heterogeneity across online tasks. Such data heterogeneity significantly degrades the model performance with severe spatial-temporal catastrophic forgetting of local and past knowledge. In this paper, we identify that the root cause of this issue lies in the inherent vulnerability and sensitivity of gradients to non-IID data. To fundamentally address this issue, we propose a gradient-free method, named Analytic Federated Continual Learning (AFCL), by deriving analytical (i.e., closed-form) solutions from frozen extracted features. In local training, our AFCL enables single-epoch learning with only a lightweight forward-propagation process for each client. In global aggregation, the server can recursively and efficiently update the global model with single-round aggregation. Theoretical analyses validate that our AFCL achieves spatio-temporal invariance of non-IID data. This ideal property implies that, regardless of how heterogeneous the data are distributed across local clients and online tasks, the aggregated model of our AFCL remains invariant and identical to that of centralized joint learning. Extensive experiments show the consistent superiority of our AFCL over state-of-the-art baselines across various benchmark datasets and settings.

==> sec/X_suppl_old.tex <==
\clearpage
\setcounter{page}{1}
% \maketitlesupplementary

% \onecolumn

\appendix


\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \caption{Description of important notations
    }
    \label{table-performance}
    % \small
        \begin{NiceTabular}{ l l }
        \toprule
        \textbf{Notations} & \textbf{Description} \\
        \midrule
        $\mathcal{X}_{k}$, $\mathcal{Y}_{k}$ & The $k$-th client's example set and label set, respectively.\\
        $\mathbf{F}_{k}$ & The $k$-th client's feature matrix.\\
        $\mathbf{\hat Y}_{k}$, $\mathbf{\check Y}_{k}$ & The $k$-th client's label matrices for known and unknown classes, respectively.\\
        $\mathbf{\hat W}_{k}$, $\mathbf{\check W}_{k}$ & The $k$-th client's regularized local weights for known and unknown classes, respectively.\\
        $\mathbf{R}_{k}$, $\mathbf{S}_{k}$ & The $k$-th client's regularized gram matrix and standard gram matrix, respectively. \\
        % $\mathbf{S}_{k}$ & The $k$-th client's standard gram matrix. \\
        $\mathbf{\widetilde R}_{k}$, $\mathbf{\widetilde S}_{k}$ & The sum of $\mathbf{R}_{k}$ and $\mathbf{S}_{k}$ for first $k$ clients, respectively. \\
        $\mathbf{G}_{k}$ & The global knowledge matrix up to the participation of the $k$-th client. \\
        $\mathbf{W}_{k}$ & The global weight up to the participation of the $k$-th client. \\
        
        \bottomrule
        \end{NiceTabular}
\end{table*}




\section{Theoretical Analysis} \label{appendix_A}


\noindent\textbf{Theorem 1:} Consider the optimization problem:
\begin{equation}
    \label{Proposition-1-1}
    \mathop{\arg\min}\limits_{\mathbf{W}} {\left\|\mathbf{Y} -\mathbf{F} \mathbf{W} \right\|}_F^2+\gamma{\left\| \mathbf{W} \right\|}_F^2,
\end{equation}
and the closed-form solution of this problem is:
\begin{equation}
    \label{Proposition-1-2}
    \mathbf{\hat W} = {({\mathbf{F}}^\top\mathbf{F}+\gamma\mathbf{I})}^{-1}{\mathbf{F}}^\top\mathbf{Y}.
\end{equation}

\noindent \textbf{\textit{Proof.}} According to \eqref{Proposition-2-1}, we can define the objective function as:
\begin{equation}
    \mathcal{L}(\mathbf{W})
    =\left\|\mathbf{Y}-\mathbf{F}\mathbf{W}\right\|_F^2 + \gamma \left\|W\right\|_F^2
    =\mathrm{Tr}\left[(\mathbf{Y}-\mathbf{F}\mathbf{W})^\top(\mathbf{Y}-\mathbf{F}\mathbf{W})\right] + \gamma \mathrm{Tr}( \mathbf{W}^\top \mathbf{W} ),
\end{equation}
which can be further expanded to:
\begin{equation}
    \mathcal{L}(\mathbf{W}) = \mathrm{Tr}(\mathbf{Y}^\top \mathbf{Y}) - 2\cdot\mathrm{Tr}(\mathbf{Y}^\top \mathbf{F} \mathbf{W}) + \mathrm{Tr}( \mathbf{W}^\top \mathbf{F}^\top \mathbf{F} \mathbf{W}) + \gamma \mathrm{Tr}(\mathbf{W}^\top \mathbf{W}).
\end{equation}
To find the minimizer $\mathbf{\hat W}$, we take the derivative of $\mathcal{L}(\mathbf{W})$, which can be calculated as follows:
\begin{equation}
\frac{ \partial \mathcal{L}(\mathbf{W}) }{\partial \mathbf{W}}
= -2\mathbf{F}^\top \mathbf{Y} + 2 \mathbf{F}^\top \mathbf{F} \mathbf{W} + 2 \gamma \mathbf{W}.
\end{equation}
By setting $\frac{ \partial \mathcal{L}(\mathbf{W}) }{\partial \mathbf{W}}=0$, we can obtain:
\begin{equation}
(\mathbf{F}^\top \mathbf{F} + \mathbf{I}) \mathbf{\hat W} = \mathbf{F}^\top \mathbf{Y}.
\end{equation}
Since $\mathbf{F}^\top \mathbf{F} + \mathbf{I}$ is positive-definite, we can obtain:
\begin{equation}
\mathbf{\hat W} =  (\mathbf{F}^\top \mathbf{F} + \mathbf{I})^{-1} \mathbf{F}^\top \mathbf{Y}.
\end{equation}

\hfill $\blacksquare$




\noindent\textbf{Inference 1:} The Global Knowledge Matrix $\mathbf{G}_{k}$ obtained using the complete dataset of the all $k$ clients $\mathcal{D}_{1:k}$ can be represented as:
\begin{equation}
\label{eq:appendix-A-inference-1-1}
\mathbf{G}_{k} = \begin{bmatrix} \sum_{i=1}^{k} ( \mathbf{F}_i^\top\mathbf{F}_i + \gamma \mathbf{I})\end{bmatrix}^{-1} \begin{bmatrix} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} + \mathbf{F}_k^\top\mathbf{\hat Y}_k  & \mathbf{F}_k^\top\mathbf{\check Y}_k   \end{bmatrix}.
\end{equation}


\noindent \textbf{\textit{Proof.}}
First, we denote the complete feature matrix and label matrix of all $k$ clients as $\mathbf{F}_{1:k}$ and $\mathbf{Y}_{1:k}$, respectively. Considering the presence of known and unknown classes in a class-incremental scenario, these matrices satisfy:
\begin{equation}
\label{eq:appendix-A-inference-1-2}
\mathbf{F}_{1:k} = \begin{bmatrix} \mathbf{F}_{1:k-1}\\ \mathbf{F}_{k} \end{bmatrix}, \quad \mathbf{Y}_{1:k} = \begin{bmatrix} \mathbf{Y}_{1:k-1} & \mathbf{0}\\ \mathbf{\hat Y}_{k} & \mathbf{\check Y}_{k} \end{bmatrix}.
\end{equation}

Therefore, we can obtain:
\begin{equation}
\label{eq:appendix-A-inference-1-3}
\begin{aligned}
    \mathbf{F}_{1:k}^\top \mathbf{F}_{1:k} &= \begin{bmatrix} \mathbf{F}_{1:k-1}^\top & \mathbf{F}_{k}^\top \end{bmatrix} \begin{bmatrix} \mathbf{F}_{1:k-1}\\ \mathbf{F}_{k} \end{bmatrix} \\
    &= \mathbf{F}_{1:k-1}^\top \mathbf{F}_{1:k-1} + \mathbf{F}_{k}^\top \mathbf{F}_{k} \\
    &= \sum\nolimits_{i=1}^k \mathbf{F}_{i}^\top \mathbf{F}_{i}.
\end{aligned}
\end{equation}
\begin{equation}
\label{eq:appendix-A-inference-1-4}
\begin{aligned}
    \mathbf{F}_{1:k}^\top \mathbf{Y}_{1:k} &= \begin{bmatrix} \mathbf{F}_{1:k-1}^\top & \mathbf{F}_{k}^\top \end{bmatrix} \begin{bmatrix} \mathbf{Y}_{1:k-1} & \mathbf{0}\\ \mathbf{\hat Y}_{k} & \mathbf{\check Y}_{k} \end{bmatrix} \\
    &= \begin{bmatrix} \mathbf{F}_{1:k-1}^\top \mathbf{Y}_{1:k-1} + \mathbf{F}_{k}^\top \mathbf{\hat Y}_{k} & \mathbf{F}_{k}^\top \mathbf{\check Y}_{k} \end{bmatrix} 
\end{aligned}
\end{equation}

By substituting \eqref{eq:appendix-A-inference-1-3} and \eqref{eq:appendix-A-inference-1-4} into \eqref{eq:Global Knowledge Matrix}, we can further derive:
\begin{equation}
\label{eq:appendix-A-inference-1-5}
\begin{aligned}
    \mathbf{G}_{k} &= \begin{bmatrix}
    \mathbf{F}_{1:k}^\top\mathbf{F}_{1:k} + \gamma \sum_{i=1}^k \mathbf{I} \end{bmatrix}^{-1} ( \mathbf{F}_{1:k}^\top\mathbf{Y}_{1:k} ) \\
    &= \begin{bmatrix}
    \sum_{i=1}^k \mathbf{F}_{i}^\top \mathbf{F}_{i} + \gamma \sum_{i=1}^k \mathbf{I} \end{bmatrix}^{-1} ( \mathbf{F}_{1:k}^\top\mathbf{Y}_{1:k} ) \\
    &= \begin{bmatrix} \sum_{i=1}^{k} ( \mathbf{F}_i^\top\mathbf{F}_i + \gamma \mathbf{I})\end{bmatrix}^{-1} \begin{bmatrix} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} + \mathbf{F}_k^\top\mathbf{\hat Y}_k  & \mathbf{F}_k^\top\mathbf{\check Y}_k   \end{bmatrix}.
\end{aligned}
\end{equation}

\hfill $\blacksquare$







\noindent\textbf{Theorem 2:} Let $\mathbf{G}_{k}$ and $\mathbf{G}_{k-1}$ represent the result of \eqref{eq:Global Knowledge Matrix} obtained using the complete dataset of the all $k$ clients $\mathcal{D}_{1:k}$ and the complete dataset of the first $k-1$ clients $\mathcal{D}_{1:k-1}$. It follows that:
\begin{equation}
\label{eq:appendix-A-theorem-2-1}
\mathbf{G}_{k} = \begin{bmatrix} \mathbf{A}_{k}  \mathbf{G}_{k-1} + \mathbf{B}_k  \mathbf{\hat W}_k & \mathbf{B}_k  \mathbf{\check W}_k \end{bmatrix},
\end{equation}
where
\begin{equation}
\label{eq:appendix-A-theorem-2-2}
\begin{cases}
\mathbf{A}_{k} = \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k (\mathbf{I} - (\mathbf{\tilde R}_{k})^{-1} \mathbf{R}_k),  \\
\mathbf{B}_{k} = \mathbf{I} - (\mathbf{R}_k)^{-1} \mathbf{\tilde R}_{k-1} (\mathbf{I} - (\mathbf{\tilde R}_{k})^{-1} \mathbf{\tilde R}_{k-1}), \\
\mathbf{\tilde R}_{k} = \sum_{i=1}^k \mathbf{R}_i, \quad
\mathbf{R}_i = \mathbf{F}_i^\top \mathbf{F}_i +\gamma\mathbf{I}.
\end{cases}
\end{equation}

\noindent \textbf{\textit{Proof.}}
According to \eqref{eq:Global Knowledge Matrix}, we can obtain that:
\begin{equation}
\label{eq:appendix-A-theorem-2-3}
\begin{aligned}
    \mathbf{G}_{k-1} 
    % &= [\sum_{i=1}^{k-1} ( \mathbf{F}_i^\top\mathbf{F}_i + \gamma \mathbf{I})]^{-1} \sum_{i=1}^{k-1} \mathbf{F}_i^\top\mathbf{Y}_i \\
    % &= (\sum_{i=1}^{k-1} \mathbf{R}_i)^{-1} \sum_{i=1}^{k-1} \mathbf{F}_i^\top\mathbf{Y}_i \\
    % &= (\mathbf{\tilde R}_{k-1})^{-1} \sum_{i=1}^{k-1} \mathbf{F}_i^\top\mathbf{Y}_i.\\
    &= \begin{bmatrix}
    \mathbf{F}_{1:k-1}^\top\mathbf{F}_{1:k-1} + \gamma \sum_{i=1}^{k-1} \mathbf{I} \end{bmatrix}^{-1} ( \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} ) \\
    &= \begin{bmatrix}\sum_{i=1}^{k-1} ( \mathbf{F}_i^\top\mathbf{F}_i + \gamma \mathbf{I})\end{bmatrix}^{-1} ( \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} ) \\
    &= (\mathbf{\tilde R}_{k-1})^{-1}( \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} ) 
\end{aligned}
\end{equation}

Then, by substituting \eqref{eq:appendix-A-theorem-2-3} into $\mathbf{A}_{k}  \mathbf{G}_{k-1}$, we can obtain:
\begin{equation}
\label{eq:appendix-A-theorem-2-4}
  \begin{aligned}
\mathbf{A}_{k}  \mathbf{G}_{k-1} &= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k (\mathbf{I} - (\mathbf{\tilde R}_{k})^{-1} \mathbf{R}_k) ] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
&= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k (\mathbf{I} - (\mathbf{R}_{k} + \mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k) ] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
&= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1}  (\mathbf{R}_k - \mathbf{R}_k(\mathbf{R}_{k} + \mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k) ] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1}\\
% &= [ (\mathbf{\tilde R}_{k-1})^{-1} - (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k (\mathbf{I} + (\mathbf{\tilde R}_{k-1} + \mathbf{R}_{k})^{-1} \mathbf{R}_k) (\mathbf{\tilde R}_{k-1})^{-1}]  \sum\nolimits_{i=1}^{k-1}\mathbf{F}_i^\top\mathbf{Y}_i \\
% &= [ (\mathbf{\tilde R}_{k-1})^{-1} - (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k (\mathbf{\tilde R}_{k-1})^{-1} - (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k (\mathbf{\tilde R}_{k})^{-1} \mathbf{R}_k (\mathbf{\tilde R}_{k-1})^{-1}]  \sum\nolimits_{i=1}^{k-1}\mathbf{F}_i^\top\mathbf{Y}_i
  \end{aligned}
\end{equation}


According to the Woodbury Matrix Identity, for any matrices $\mathbf{A}\in\mathbb{R}^{n\times n}$, $\mathbf{B}\in\mathbb{R}^{n\times m}$, $\mathbf{E}\in\mathbb{R}^{m\times m}$, and $\mathbf{D}\in\mathbb{R}^{m\times n}$, the following equation holds consistently:
\begin{equation}
\label{eq:appendix-A-theorem-2-5}
(\mathbf{A}+\mathbf{B}\mathbf{E}\mathbf{D})^{-1}=\mathbf{A}^{-1}-\mathbf{A}^{-1}\mathbf{B}(\mathbf{E}^{-1}+\mathbf{D}\mathbf{A}^{-1}\mathbf{B})^{-1}\mathbf{D}\mathbf{A}^{-1}.
\end{equation}


Subsequently, based on \eqref{eq:appendix-A-theorem-2-5}, we substitute both $\mathbf{B}$ and $\mathbf{D}$ with $\mathbf{I}$. This adjustment allows us to derive:
\begin{equation}
\label{eq:appendix-A-theorem-2-6}
(\mathbf{A}+\mathbf{E})^{-1}=\mathbf{A}^{-1}-\mathbf{A}^{-1}(\mathbf{A}^{-1}+\mathbf{E}^{-1})^{-1}\mathbf{A}^{-1}
\end{equation}

Further, it can be obtained:
\begin{equation}
\label{eq:appendix-A-theorem-2-7}
\mathbf{A}^{-1}(\mathbf{A}^{-1}+\mathbf{E}^{-1})^{-1}\mathbf{A}^{-1} = \mathbf{A}^{-1} - (\mathbf{A}+\mathbf{E})^{-1}.
\end{equation}

By replacing $\mathbf{A}^{-1}$ and $\mathbf{E}^{-1}$ in \eqref{eq:appendix-A-theorem-2-7} with $\mathbf{R}_k$ and $\mathbf{\tilde R}_{k-1}$ respectively, yields:
\begin{equation}
\label{eq:appendix-A-theorem-2-8}
\mathbf{R}_k(\mathbf{R}_k+\mathbf{\tilde R}_{k-1})^{-1}\mathbf{R}_k = \mathbf{R}_k - ( (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{R}_k)^{-1} )^{-1}
\end{equation}



Incorporating \eqref{eq:appendix-A-theorem-2-8} into \eqref{eq:appendix-A-theorem-2-4}, we can find:
\begin{equation}
\label{eq:appendix-A-theorem-2-9}
  \begin{aligned}
\mathbf{A}_{k}  \mathbf{G}_{k-1} &= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1}  (\mathbf{R}_k - \mathbf{R}_k(\mathbf{R}_{k} + \mathbf{\tilde R}_{k-1})^{-1} \mathbf{R}_k) ] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1}\\
&= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1}  (\mathbf{R}_k - \mathbf{R}_k + ( (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{R}_k)^{-1} )^{-1} )] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
&= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1}  ( (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{R}_k)^{-1} )^{-1} ] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1}
  \end{aligned}
\end{equation}



\noindent Subsequently, replacing $\mathbf{A}$ and $\mathbf{E}$ in \eqref{eq:appendix-A-theorem-2-5} with $\mathbf{M}_i^\mathrm{r}$ and $\mathbf{M}_j^\mathrm{r}$ respectively, yields:
\begin{equation}
\label{eq:appendix-A-theorem-2-10}
(\mathbf{\tilde R}_{k-1})^{-1} ( (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{R}_k)^{-1} )^{-1} (\mathbf{\tilde R}_{k-1})^{-1} = (\mathbf{\tilde R}_{k-1})^{-1} - (\mathbf{\tilde R}_{k-1}+\mathbf{R}_k)^{-1}
\end{equation}


Similarly, by incorporating \eqref{eq:appendix-A-theorem-2-10} into \eqref{eq:appendix-A-theorem-2-9}, we can obtain:
\begin{equation}
\label{eq:appendix-A-theorem-2-11}
  \begin{aligned}
\mathbf{A}_{k}  \mathbf{G}_{k-1} &= [ \mathbf{I} - (\mathbf{\tilde R}_{k-1})^{-1}  ( (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{R}_k)^{-1} )^{-1} ] (\mathbf{\tilde R}_{k-1})^{-1} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
&= [ (\mathbf{\tilde R}_{k-1})^{-1} - (\mathbf{\tilde R}_{k-1})^{-1}  ( (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{R}_k)^{-1} )^{-1} (\mathbf{\tilde R}_{k-1})^{-1}]  \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
&= [ (\mathbf{\tilde R}_{k-1})^{-1} - (\mathbf{\tilde R}_{k-1})^{-1} + (\mathbf{\tilde R}_{k-1}+\mathbf{R}_k)^{-1}]  \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
&= (\mathbf{\tilde R}_{k})^{-1}  \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} \\
  \end{aligned}
\end{equation}


Similarly, we can obtain:
\begin{equation}
\label{eq:appendix-A-theorem-2-12}
\mathbf{B}_k  \mathbf{\hat W}_k= (\mathbf{\tilde R}_{k})^{-1} \mathbf{F}_k^\top \mathbf{\hat Y}_j,
\end{equation}
\begin{equation}
\label{eq:appendix-A-theorem-2-13}
\mathbf{B}_k  \mathbf{\check W}_k = (\mathbf{\tilde R}_{k})^{-1} \mathbf{F}_k^\top \mathbf{\check Y}_j.
\end{equation}


By substituting \eqref{eq:appendix-A-theorem-2-11}, \eqref{eq:appendix-A-theorem-2-12}, and \eqref{eq:appendix-A-theorem-2-13} into \eqref{eq:appendix-A-theorem-2-1}, we can further derive:
\begin{equation}
\label{eq:appendix-A-theorem-2-14}
\begin{aligned}
    \mathbf{G}_{k} &= \begin{bmatrix} \mathbf{A}_{k}  \mathbf{G}_{k-1} + \mathbf{B}_k  \mathbf{\hat W}_k & \mathbf{B}_k  \mathbf{\check W}_k \end{bmatrix} \\
    &= \begin{bmatrix} (\mathbf{\tilde R}_{k})^{-1}  \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} + (\mathbf{\tilde R}_{k})^{-1} \mathbf{F}_k^\top \mathbf{\hat Y}_j & (\mathbf{\tilde R}_{k})^{-1} \mathbf{F}_k^\top \mathbf{\check Y}_j \end{bmatrix} \\
    &= (\mathbf{\tilde R}_{k})^{-1} \begin{bmatrix} \mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} + \mathbf{F}_k^\top \mathbf{\hat Y}_j & \mathbf{F}_k^\top \mathbf{\check Y}_j \end{bmatrix} \\
    &=\begin{bmatrix} \sum_{i=1}^{k} ( \mathbf{F}_i^\top\mathbf{F}_i + \gamma \mathbf{I})\end{bmatrix}^{-1} \begin{bmatrix}\mathbf{F}_{1:k-1}^\top\mathbf{Y}_{1:k-1} + \mathbf{F}_k^\top\mathbf{\hat Y}_k  & \mathbf{F}_k^\top\mathbf{\check Y}_k   \end{bmatrix}.
\end{aligned}
\end{equation}

It is evident that the result obtained from \eqref{eq:appendix-A-theorem-2-1}, i.e., \eqref{eq:appendix-A-theorem-2-14}, is equivalent to the result of \eqref{eq:appendix-A-inference-1-1} in \textbf{Inference 1}, thereby confirming the correctness of our iterative update method for the Global Knowledge Matrix.

\hfill $\blacksquare$


\noindent\textbf{Theorem 3:} Let $\mathbf{W}_{k}$ and $\mathbf{G}_{k}$ represent the results of \eqref{Motivation-1} and \eqref{eq:Global Knowledge Matrix} obtained using the complete dataset of the all $k$ clients $\mathcal{D}_{1:k}$, while $\mathbf{\hat W}_{k}$ and $\mathbf{\check W}_{k}$ represent the results of \eqref{eq:client-3} and \eqref{eq:client-4} respectively using local datasets of the $k$-th client $\mathcal{D}_{k}$. It follows that:
\begin{equation}
\label{eq:appendix-A-theorem-3-1}
  \begin{aligned}
\mathbf{W}_k=[\mathbf{\tilde R}_{k} - (k-1)\gamma \mathbf{I}]^{-1} \mathbf{\tilde R}_{k} \mathbf{G}_{k},
\end{aligned}
\end{equation}
where
\begin{equation}
\label{eq:appendix-A-theorem-3-2}
\mathbf{\tilde R}_{k} = \sum_i^k \mathbf{R}_i, \quad
\mathbf{R}_i = \mathbf{F}_i^\top \mathbf{F}_i +\gamma\mathbf{I}.
\end{equation}

\noindent \textbf{\textit{Proof.}} According to \eqref{eq:Global Knowledge Matrix}, and \eqref{eq:appendix-A-theorem-3-2}, we can obtain that:
% \begin{equation}
%     \label{eq:appendix-A-theorem-3-3}
%     \begin{aligned}
%         \mathbf{W}_k &= {({\mathbf{F}}^\top_{1:k}  \mathbf{F}_{1:k}+\gamma\mathbf{I})}^{-1}({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}) \\
%         &= ( \sum\nolimits_{i=1}^k {\mathbf{F}}^\top_k  \mathbf{F}_k + \gamma\mathbf{I}) ^{-1} ({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}) \\
%         &= [ \mathbf{\tilde R}_k - (k-1)\gamma\mathbf{I} ] ^{-1} ({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}),
%     \end{aligned}
% \end{equation}
\begin{equation}
    \label{eq:appendix-A-theorem-3-4}
    \begin{aligned}
    \mathbf{G}_k 
    &= \begin{bmatrix} \mathbf{F}_{1:k}^\top\mathbf{F}_{1:k} + \gamma \sum_{i=1}^k \mathbf{I} \end{bmatrix}^{-1} ( \mathbf{F}_{1:k}^\top\mathbf{Y}_{1:k} ) \\
    &= \begin{bmatrix} \sum\nolimits_{i=1}^k {\mathbf{F}}^\top_k {\mathbf{F}}_k + \gamma \sum_{i=1}^k \mathbf{I} \end{bmatrix}^{-1} ( \mathbf{F}_{1:k}^\top\mathbf{Y}_{1:k} ) \\
    &= \begin{bmatrix} \sum\nolimits_{i=1}^k ({\mathbf{F}}^\top_k {\mathbf{F}}_k + \gamma \mathbf{I}) \end{bmatrix}^{-1} ( \mathbf{F}_{1:k}^\top\mathbf{Y}_{1:k} ) \\
    &= ( \mathbf{\tilde R}_k ) ^{-1} ({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}).
    \end{aligned}
\end{equation}

% Therefore, we can further obtain:
% \begin{equation}
%     \begin{aligned}
%         &[ \mathbf{\tilde R}_k - (k-1)\gamma\mathbf{I} ] \mathbf{\hat W}_k = \mathbf{\tilde R}_k \mathbf{G}_k \\
%         \Rightarrow &  \mathbf{W}_k = [ \mathbf{\tilde R}_k - (k-1)\gamma\mathbf{I} ]^{-1}\mathbf{\tilde R}_k \mathbf{G}_k.
%     \end{aligned}
% \end{equation}


By substituting \eqref{eq:appendix-A-theorem-3-4} into \eqref{eq:appendix-A-theorem-3-1}, we can further derive:
\begin{equation}
    \label{eq:appendix-A-theorem-3-5}
    \begin{aligned}
    \mathbf{W}_k
    &=[\mathbf{\tilde R}_{k} - (k-1)\gamma \mathbf{I}]^{-1} \mathbf{\tilde R}_{k} \mathbf{G}_{k} \\
    &=[\mathbf{\tilde R}_{k} - (k-1)\gamma \mathbf{I}]^{-1} \mathbf{\tilde R}_{k} ( \mathbf{\tilde R}_k ) ^{-1} ({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}) \\
    &=[\mathbf{\tilde R}_{k} - (k-1)\gamma \mathbf{I}]^{-1} ({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}) \\
    &=( \sum\nolimits_{i=1}^k {\mathbf{F}}^\top_k  \mathbf{F}_k + \gamma\mathbf{I}) ^{-1} ({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k}) \\
    &={({\mathbf{F}}^\top_{1:k}  \mathbf{F}_{1:k}+\gamma\mathbf{I})}^{-1}({\mathbf{F}}^\top_{1:k} \mathbf{Y}_{1:k})
    \end{aligned}
\end{equation}

It is evident that the result derived from \eqref{eq:server-5}, i.e., \eqref{eq:appendix-A-theorem-3-1}, is equivalent to the centralized result of \eqref{Motivation-2} obtained using the complete dataset of all $k$ clients $\mathcal{D}_{1:k}$, thereby validating the correctness of our scheme.

\hfill $\blacksquare$


In summary, the global model $\mathbf{W}_k$ obtained by our AFCL scheme through federated learning is fully equivalent to the result derived from centralized training using the complete dataset.

























\clearpage


% 前一版的证明：

\noindent\textbf{Proposition 1:} Consider the optimization problem:
\begin{equation}
    \label{Proposition-1-1}
    \mathop{\arg\min}\limits_{\mathbf{W}} {\left\|\mathbf{Y} -\mathbf{X} \mathbf{W} \right\|}_F^2,
\end{equation}
and the closed-form solution of this problem is:
\begin{equation}
    \label{Proposition-1-2}
    \mathbf{\hat W} = \mathbf{X}^{\dagger} \mathbf{ Y}.
\end{equation}

\noindent \textbf{\textit{Proof.}}
Let us define its objective function as:
\begin{equation}
    \mathcal{L}(\mathbf{W})=\left\|\mathbf{Y}-\mathbf{X}\mathbf{W}\right\|_F^2=\mathrm{Tr}\left[(\mathbf{Y}-\mathbf{X}\mathbf{W})^\top(\mathbf{Y}-\mathbf{X}\mathbf{W})\right],
\end{equation}
where $\mathrm{Tr}( \cdot )$ denotes the trace of a matrix. To find the minimizer $\mathbf{\hat W}$, we take the derivative of $\mathcal{L}(\mathbf{W})$, which can be calculated as follows:
\begin{equation}
\frac{ \partial \mathcal{L}(\mathbf{W}) }{\partial \mathbf{W}}
=-2\mathbf{X}^\top (\mathbf{Y} -  \mathbf{X}\mathbf{W} )
\end{equation}

\noindent By setting $\frac{ \partial \mathcal{L}(\mathbf{W}) }{\partial \mathbf{W}}=0$ we can obtain:
\begin{equation}
\mathbf{X}^\top \mathbf{X} \mathbf{\hat W} = \mathbf{X}^\top \mathbf{Y}.
\end{equation}

\noindent Since $\mathbf{X}^\top \mathbf{X}$ may be singular or $\mathbf{X}$ may be rank-deficient, we utilize the MP inverse to obtain the least-squares solution:
\begin{equation}
    \mathbf{\hat W} = \mathbf{X}^{\dagger} \mathbf{ Y}.
\end{equation}

\hfill $\blacksquare$


\noindent\textbf{Proposition 2:} Consider the optimization problem:
\begin{equation}
    \label{Proposition-2-1}
    \mathop{\arg\min}\limits_{\mathbf{W}} {\left\|\mathbf{Y} -\mathbf{X} \mathbf{W} \right\|}_F^2+\gamma{\left\| \mathbf{W} \right\|}_F^2,
\end{equation}
and the closed-form solution of this problem is:
\begin{equation}
    \label{Proposition-2-2}
    \mathbf{\hat W} = {({\mathbf{X}}^\top\mathbf{X}+\gamma\mathbf{I})}^{-1}{\mathbf{X}}^\top\mathbf{Y}.
\end{equation}

\noindent \textbf{\textit{Proof.}} According to \eqref{Proposition-2-1}, we can define the objective function as:
\begin{equation}
    \mathcal{L}(\mathbf{W})
    =\left\|\mathbf{Y}-\mathbf{X}\mathbf{W}\right\|_F^2 + \gamma \left\|W\right\|_F^2
    =\mathrm{Tr}\left[(\mathbf{Y}-\mathbf{X}\mathbf{W})^\top(\mathbf{Y}-\mathbf{X}\mathbf{W})\right] + \gamma \mathrm{Tr}( \mathbf{W}^\top \mathbf{W} ),
\end{equation}
which can be further expanded to:
\begin{equation}
    \mathcal{L}(\mathbf{W}) = \mathrm{Tr}(\mathbf{Y}^\top \mathbf{Y}) - 2\cdot\mathrm{Tr}(\mathbf{Y}^\top \mathbf{X} \mathbf{W}) + \mathrm{Tr}( \mathbf{W}^\top \mathbf{X}^\top \mathbf{X} \mathbf{W}) + \gamma \mathrm{Tr}(\mathbf{W}^\top \mathbf{W}).
\end{equation}
To find the minimizer $\mathbf{\hat W}$, we take the derivative of $\mathcal{L}(\mathbf{W})$, which can be calculated as follows:
\begin{equation}
\frac{ \partial \mathcal{L}(\mathbf{W}) }{\partial \mathbf{W}}
= -2\mathbf{X}^\top \mathbf{Y} + 2 \mathbf{X}^\top \mathbf{X} \mathbf{W} + 2 \gamma \mathbf{W}.
\end{equation}
By setting $\frac{ \partial \mathcal{L}(\mathbf{W}) }{\partial \mathbf{W}}=0$, we can obtain:
\begin{equation}
(\mathbf{X}^\top \mathbf{X} + \mathbf{I}) \mathbf{\hat W} = \mathbf{X}^\top \mathbf{Y}.
\end{equation}
Since $\mathbf{X}^\top \mathbf{X} + \mathbf{I}$ is positive-definite, we can obtain:
\begin{equation}
\mathbf{\hat W} =  (\mathbf{X}^\top \mathbf{X} + \mathbf{I})^{-1} \mathbf{X}^\top \mathbf{Y}.
\end{equation}

\hfill $\blacksquare$

\clearpage











To illustrate this process clearly, we first consider a scenario with two clients, denoted as client $i$ and client $j$, where the complete dataset is $\mathbf{X} = \begin{bmatrix} \mathbf{X}_i \\ \mathbf{X}_j\end{bmatrix}$ and $\mathbf{Y} = \begin{bmatrix} \mathbf{Y}_i & \textbf{0} \\ \mathbf{\bar Y}_j & \mathbf{\tilde Y}_j  \end{bmatrix}$. 

% For the client $i$, the model weights can be computed as:
% \begin{small} 
% \begin{equation*}
%    \mathbf{W}_i^\mathrm{r} = (\mathbf{M}_i^\mathrm{r})^{-1}\mathbf{X}_i^\top\mathbf{ Y}_i,
%    \mathbf{M}_i^\mathrm{r} = \mathbf{X}_i^\top \mathbf{X}_i +\gamma\mathbf{I},
% \end{equation*}
% \end{small} 

% For the client $j$, the model weights can be computed as:
% \begin{small} 
% \begin{equation*}
%    \hat{\mathbf{W}}_j^\mathrm{r} =(\mathbf{M}_j^\mathrm{r})^{-1}\mathbf{X}_k^\top\mathbf{\bar Y}_j, 
%    \check{\mathbf{W}}_j^\mathrm{r} =(\mathbf{M}_j^\mathrm{r})^{-1}\mathbf{X}_k^\top\mathbf{\tilde Y}_j,
%    \mathbf{M}_j^\mathrm{r} = \mathbf{X}_j^\top \mathbf{X}_j +\gamma\mathbf{I}. 
% \end{equation*}
% \end{small} 



% Moreover, we can further extend the model aggregation from two clients to multiple clients.




\noindent \textbf{Lemma 1:} For $\mathbf{X}=\begin{bmatrix}\mathbf{X}_i\\\mathbf{X}_j\end{bmatrix}$ , composed of two matrices $\mathbf{X}_{i}$ and $\mathbf{X}_{j}$ both satisfying column full rank, its MP inverse $\mathbf{X}_{k}^{\dagger}$ adheres to the following partition:
\begin{equation}
\label{eq:Lema_1}
  \mathbf{X}^{\dagger}=\begin{bmatrix}\bar{\mathbf{U}}&\bar{\mathbf{V}}\end{bmatrix},
\end{equation}
where
\begin{equation}
\label{eq:Lema_2}
\begin{cases}
\mathbf{\bar{U}} = \mathbf{X}_i^\dagger - \mathbf{M}_i^{-1} \mathbf{M}_j \mathbf{X}_i^\dagger - \mathbf{M}_i^{-1} \mathbf{M}_j (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_j \mathbf{X}_i^\dagger, \\
\mathbf{\bar{V}} = \mathbf{X}_j^\dagger - \mathbf{M}_j^{-1} \mathbf{M}_i \mathbf{X}_j^\dagger - \mathbf{M}_j^{-1} \mathbf{M}_i (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_i \mathbf{X}_j^\dagger, \\
\mathbf{M}_i = \mathbf{X}_i^\top \mathbf{X}_i, \quad \quad \mathbf{M}_j = \mathbf{X}_j^\top \mathbf{X}_j.
\end{cases}
\end{equation}



\noindent \textbf{\textit{Proof.}} Existing research on MP inverse partitioning \cite{AL_7} has demonstrated that the MP inverse of any matrix $\mathbf{A}=[\mathbf{U}\quad\mathbf{V}]$ can be expressed as follows:


\begin{equation}
\label{eq:appendix1_1}
  \mathbf{A}^\dagger = [\mathbf{U}\quad \mathbf{V}]^\dagger
     = \begin{bmatrix}\mathbf{U}^\dagger-\mathbf{U}^\dagger \mathbf{V}\mathbf{M}^\dagger-\mathbf{U}^\dagger \mathbf{V}(\mathbf{I}-\mathbf{M}^\dagger \mathbf{M})\mathbf{K}\mathbf{V}^*\mathbf{U}^\dagger*\mathbf{U}^\dagger(\mathbf{I}-\mathbf{V}\mathbf{M}^\dagger)\\\mathbf{V}^\dagger-\mathbf{V}^\dagger \mathbf{U}\tilde{\mathbf{M}}^\dagger-\mathbf{V}^\dagger \mathbf{U}(\mathbf{I}-\tilde{\mathbf{M}}^\dagger\tilde{\mathbf{M}})\tilde{\mathbf{K}}\mathbf{U}^*\mathbf{V}^\dagger*\mathbf{V}^\dagger(\mathbf{I}-\mathbf{U}\tilde{\mathbf{M}}^\dagger)\end{bmatrix},
\end{equation}
where

\begin{equation}
\label{eq:appendix1_2}
\begin{cases}
\mathbf{M}=(\mathbf{I}-\mathbf{U}\mathbf{U}^\dagger)\mathbf{V}\\
\mathbf{\tilde{M}}=(\mathbf{I}-\mathbf{V}\mathbf{V}^\dagger)\mathbf{U}
\end{cases},\quad
\begin{cases}
\mathbf{K}=\begin{bmatrix}
\mathbf{I}+(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})\mathbf{V}^*\mathbf{U}^\dagger*\mathbf{U}^\dagger\mathbf{V}(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})
\end{bmatrix}^{-1}\\
\mathbf{\tilde{K}}=\begin{bmatrix}
\mathbf{I}+(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})\mathbf{U}^*\mathbf{V}^\dagger*\mathbf{V}^\dagger\mathbf{U}(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})
\end{bmatrix}^{-1}
\end{cases}.
\end{equation}


\noindent Furthermore, by substituting $\mathbf{X}_i^\top $ for $\mathbf{U}$ and $\mathbf{X}_j^\top $ for $\mathbf{V}$, (\ref{eq:appendix1_1}) and (\ref{eq:appendix1_2}) can be transformed as follows:

\begin{equation}
\label{eq:appendix1_3}
  \mathbf{X}^{\dagger}=\begin{bmatrix}\mathbf{X}_{i}\\\mathbf{X}_{j}\end{bmatrix}^{\dagger}=\begin{bmatrix}\mathbf{X}_{i}^{\dagger\top}-\mathbf{X}_{i}^{\dagger\top}\mathbf{X}_{j}^{\top}\mathbf{M}^{\dagger}-\mathbf{X}_{i}^{\dagger\top}\mathbf{X}_{j}^{\top}(\mathbf{I}-\mathbf{M}^{\dagger}\mathbf{M})\mathbf{K}\mathbf{X}_{j}\mathbf{X}_{i}^{\dagger}\mathbf{X}_{i}^{\dagger\top}(\mathbf{I}-\mathbf{X}_{j}^{\top}\mathbf{M}^{\dagger}),\\
\mathbf{X}_{j}^{\dagger\top}-\mathbf{X}_{j}^{\dagger\top}\mathbf{X}_{i}^{\top}\tilde{\mathbf{M}}^{\dagger}-\mathbf{X}_{j}^{\dagger\top}\mathbf{X}_{i}^{\top}(\mathbf{I}-\tilde{\mathbf{M}}^{\dagger}\tilde{\mathbf{M}})\tilde{\mathbf{K}}\mathbf{X}_{i}\mathbf{X}_{j}^{\dagger}\mathbf{X}_{j}^{\dagger\top}(\mathbf{I}-\mathbf{X}_{i}^{\top}\tilde{\mathbf{M}}^{\dagger})\end{bmatrix}^{\top},
\end{equation}
where

\begin{equation}
\label{eq:appendix1_4}
  \begin{cases}
\mathbf{M}=(\mathbf{I}-\mathbf{X}_i^\top\mathbf{X}_i^{\dagger\top})\mathbf{X}_j^\top \\
\mathbf{\tilde{M}}=(\mathbf{I}-\mathbf{X}_j^\top\mathbf{X}_j^{\dagger\top})\mathbf{X}_i^\top
\end{cases},\quad
\begin{cases}
\mathbf{K}=\begin{bmatrix}
\mathbf{I}+(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})\mathbf{X}_j\mathbf{X}_i^\dagger\mathbf{X}_i^\dagger\top\mathbf{X}_j^\top(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})
\end{bmatrix}^{-1} \\
\mathbf{\tilde{K}}=\begin{bmatrix}
\mathbf{I}+(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})\mathbf{X}_i\mathbf{X}_j^\dagger\mathbf{X}_j^\dagger\top\mathbf{X}_i^\top(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})
\end{bmatrix}^{-1}
\end{cases}.
\end{equation}

\noindent Given that both $\mathbf{X}_i$ and $\mathbf{X}_j$ possess column full rank, their MP inverses can be computed as:

\begin{equation}
\label{eq:appendix1_5}
\mathbf{X}_i^\dagger=(\mathbf{X}_i^\top\mathbf{X}_i)^{-1}\mathbf{X}_i^\top,
\quad\mathbf{X}_j^\dagger=(\mathbf{X}_j^\top\mathbf{X}_j)^{-1}\mathbf{X}_j^\top.
\end{equation}


\noindent Substituting (\ref{eq:appendix1_5}) into (\ref{eq:appendix1_4}) yields that $\mathbf{M}$ and $\mathbf{\tilde{M}}$ can be computed as:
\begin{equation}
\label{eq:appendix1_6}
  \begin{cases}
\mathbf{M}=(\mathbf{I}-\mathbf{X}_i^\top\mathbf{X}_i^{\dagger\top})\mathbf{X}_j^\top = (\mathbf{I}-\mathbf{X}_i^\top\mathbf{X}_i(\mathbf{X}_i^\top\mathbf{X}_i)^{-1})\mathbf{X}_j^\top=\mathbf{0} \\
\mathbf{\tilde{M}}=(\mathbf{I}-\mathbf{X}_j^\top\mathbf{X}_j^{\dagger\top})\mathbf{X}_i^\top = (\mathbf{I}-\mathbf{X}_j^\top\mathbf{X}_j(\mathbf{X}_j^\top\mathbf{X}_j)^{-1})\mathbf{X}_i^\top=\mathbf{0}
\end{cases}
\end{equation}


\noindent Furthermore, $\mathbf{K}$ and $\mathbf{\tilde{K}}$ can be calculated as:
\begin{equation}
\label{eq:appendix1_7}
\begin{cases}
\mathbf{K}=\begin{bmatrix}
\mathbf{I}+(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})\mathbf{X}_j\mathbf{X}_i^\dagger\mathbf{X}_i^\dagger\top\mathbf{X}_j^\top(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})
\end{bmatrix}^{-1}=(\mathbf{I}+\mathbf{X}_{j}\mathbf{X}_{i}^{\dagger}\mathbf{X}_{i}^{\dagger\top}\mathbf{X}_{j}^{\top})^{-1}\\
\mathbf{\tilde{K}}=\begin{bmatrix}
\mathbf{I}+(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})\mathbf{X}_i\mathbf{X}_j^\dagger\mathbf{X}_j^\dagger\top\mathbf{X}_i^\top(\mathbf{I}-\mathbf{M}^\dagger\mathbf{M})
\end{bmatrix}^{-1}=(\mathbf{I}+\mathbf{X}_{i}\mathbf{X}_{j}^{\dagger}\mathbf{X}_{j}^{\dagger\top}\mathbf{X}_{i}^{\top})^{-1}
\end{cases}
\end{equation}

\noindent Meanwhile, (\ref{eq:appendix1_3}) can also be reduced to:
\begin{equation}
\label{eq:appendix1_8}
\mathbf{X}^\dagger=\begin{bmatrix}
\mathbf{X}_i^{\dagger\top}-\mathbf{X}_i^{\dagger\top}\mathbf{X}_j^{\top}\mathbf{K}\mathbf{X}_j\mathbf{X}_i^{\dagger}\mathbf{X}_i^{\dagger\top} \\
\mathbf{X}_j^{\dagger\top}-\mathbf{X}_j^{\dagger\top}\mathbf{X}_i^{\top}\mathbf{K}\mathbf{X}_i\mathbf{X}_j^{\dagger}\mathbf{X}_j^{\dagger\top}
\end{bmatrix}^\top
\end{equation}


\noindent Subsequently, applying the Woodbury Matrix Identity reveals that for conformable matrices $\mathbf{A}\in\mathbb{R}^{n\times n}$, $\mathbf{B}\in\mathbb{R}^{n\times m}$, $\mathbf{E}\in\mathbb{R}^{m\times m}$, and $\mathbf{D}\in\mathbb{R}^{m\times n}$, (\ref{eq:appendix1_8}) consistently holds.
\begin{equation}
\label{eq:appendix1_9}
(\mathbf{A}+\mathbf{B}\mathbf{E}\mathbf{D})^{-1}=\mathbf{A}^{-1}-\mathbf{A}^{-1}\mathbf{B}(\mathbf{E}^{-1}+\mathbf{D}\mathbf{A}^{-1}\mathbf{B})^{-1}\mathbf{D}\mathbf{A}^{-1}.
\end{equation}

\noindent By substituting $\mathbf{A}$ with $\mathbf{I}$, $\mathbf{I}$ with $\mathbf{X}_j$, $\mathbf{E}$ with $\mathbf{X}_i^\dagger \mathbf{X}_i^{\dagger\top}$, and $\mathbf{D}$ with $\mathbf{X}_j^\top$ in (\ref{eq:appendix1_9}), we derive the following result:
\begin{equation}
\label{eq:appendix1_10}
\mathbf{K}=\mathbf{I}-\mathbf{X}_j(\mathbf{X}_i^\top\mathbf{X}_i+\mathbf{X}_j^\top\mathbf{X}_j)^{-1}\mathbf{X}_j^\top.
\end{equation}

\noindent Similarly, we can obtain 
\begin{equation}
\label{eq:appendix1_11}
\mathbf{\tilde{K}}=\mathbf{I}-\mathbf{X}_i(\mathbf{X}_i^\top \mathbf{X}_i+\mathbf{X}_j^\top \mathbf{X}_j)^{-1}\mathbf{X}_i^\top.
\end{equation}

\noindent Let $X^\dagger=\begin{bmatrix}\bar{U}&\bar{V}\end{bmatrix}$, we have
\begin{equation}
\label{eq:appendix1_12}
\begin{cases}
\mathbf{\bar{U}}=(\mathbf{X}_i^{\dagger\top}-\mathbf{X}_i^{\dagger\top}\mathbf{X}_j^{\top}\mathbf{K}\mathbf{X}_j\mathbf{X}_i^{\dagger}\mathbf{X}_i^{\dagger\top})^{\top}=\mathbf{X}_i^{\dagger}-\mathbf{X}_i^{\dagger}\mathbf{X}_i^{\dagger\top}\mathbf{X}_j^{\top}\mathbf{K}^{\top}\mathbf{X}_j\mathbf{X}_i^{\dagger} \\
\mathbf{\bar{V}}=\left(\mathbf{X}_j^{\dagger\top}-\mathbf{X}_j^{\dagger\top}\mathbf{X}_i^{\top}\mathbf{\tilde{K}}\mathbf{X}_i\mathbf{X}_j^{\dagger}\mathbf{X}_j^{\dagger\top}\right)^{\top}=\mathbf{X}_j^{\dagger}-\mathbf{X}_j^{\dagger}\mathbf{X}_j^{\dagger\top}\mathbf{X}_i^{\top}\mathbf{\tilde{K}}^{\top}\mathbf{X}_i\mathbf{X}_j^{\dagger}
\end{cases}
\end{equation}

\noindent By substituting $\mathbf{K}$ and $\mathbf{\tilde{K}}$ from (\ref{eq:appendix1_10}) and (\ref{eq:appendix1_11}) into (\ref{eq:appendix1_12}), we can obtained:
\begin{equation}
\label{eq:appendix1_13}
\begin{cases}
\mathbf{\bar{U}}=\mathbf{X}_i^\dagger-\mathbf{X}_i^\dagger\mathbf{X}_i^{\dagger\top}\mathbf{X}_j^\top\left(\mathbf{I}-\mathbf{X}_j(\mathbf{X}_i^\top\mathbf{X}_i+\mathbf{X}_j^\top\mathbf{X}_j)^{-1}\mathbf{X}_j^\top\right)^\top\mathbf{X}_j\mathbf{X}_i^\dagger \\
\mathbf{\bar{V}}=\mathbf{X}_j^\dagger-\mathbf{X}_j^\dagger\mathbf{X}_j^\dagger\top\mathbf{X}_i^\top\left(\mathbf{I}-\mathbf{X}_i(\mathbf{X}_i^\top\mathbf{X}_i+\mathbf{X}_j^\top\mathbf{X}_j)^{-1}\mathbf{X}_i^\top\right)^\top\mathbf{X}_i\mathbf{X}_j^\dagger
\end{cases}
\end{equation}

\noindent That is,
\begin{equation}
\label{eq:appendix1_14}
\begin{cases}
\mathbf{\bar{U}} = \mathbf{X}_i^\dagger - \mathbf{X}_i^\dagger \mathbf{X}_i^{\dagger\top} \mathbf{X}_j^\top \mathbf{X}_j \mathbf{X}_i^\dagger - \mathbf{X}_i^\dagger \mathbf{X}_i^\dagger \mathbf{X}_j^\top \mathbf{X}_j (\mathbf{X}_i^\top \mathbf{X}_i + \mathbf{X}_j^\top \mathbf{X}_j)^{-1} \mathbf{X}_j^\top \mathbf{X}_j \mathbf{X}_i^\dagger \\
\mathbf{\bar{V}} = \mathbf{X}_j^\dagger - \mathbf{X}_j^\dagger \mathbf{X}_j^{\dagger\top} \mathbf{X}_i^\top \mathbf{X}_i \mathbf{X}_j^\dagger - \mathbf{X}_j^\dagger \mathbf{X}_j^\dagger \mathbf{X}_i^\top \mathbf{X}_i (\mathbf{X}_i^\top \mathbf{X}_i + \mathbf{X}_j^\top \mathbf{X}_j)^{-1} \mathbf{X}_i^\top \mathbf{X}_i \mathbf{X}_j^\dagger
\end{cases}
\end{equation}

\noindent We denote
\begin{equation}
\label{eq:appendix1_15}
\left.\left\{\begin{matrix}
\mathbf{M}_i=\mathbf{X}_i^\top \mathbf{X}_i \\
\mathbf{M}_j=\mathbf{X}_j^\top \mathbf{X}_j
\end{matrix}\right.\right., \left\{\begin{matrix}
\mathbf{R}_i=\mathbf{M}_i^{-1} \\
\mathbf{R}_j=\mathbf{M}_j^{-1}
\end{matrix}.\right.
\end{equation}

\noindent Consequently, (\ref{eq:appendix1_14}) can be rewritten as:
\begin{equation}
\label{eq:appendix1_16}
\begin{cases}
\mathbf{\bar{U}} = \left[\mathbf{I} - \mathbf{R}_i \mathbf{M}_j - \mathbf{R}_i \mathbf{M}_j (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_j \right] \mathbf{X}_i^\dagger \\
\mathbf{\bar{V}} = \left[\mathbf{I} - \mathbf{R}_j \mathbf{M}_i - \mathbf{R}_j \mathbf{M}_i (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_i \right] \mathbf{X}_j^\dagger
\end{cases}
\end{equation}

\noindent Thus, 
\begin{equation}
\label{eq:appendix1_17}
\mathbf{X}^\dagger = \begin{bmatrix} \mathbf{X}_i \\ \mathbf{X}_j \end{bmatrix}^\dagger = 
\begin{bmatrix} \mathbf{\bar{U}} & \mathbf{\bar{V}} \end{bmatrix}
\end{equation}

\noindent Based on (\ref{eq:appendix1_15}), (\ref{eq:appendix1_16}), and (\ref{eq:appendix1_17}), the proof is completed. 

\hfill $\blacksquare$


% \clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\noindent \textbf{Proposition 3.} Let ${\mathbf{W}} = \mathbf{X}^\dagger \mathbf{Y}$, $\mathbf{X} = \begin{bmatrix} \mathbf{X}_i \\ \mathbf{X}_j\end{bmatrix}$ and $\mathbf{Y} = \begin{bmatrix} \mathbf{Y}_i & \textbf{0} \\ \mathbf{\bar Y}_j & \mathbf{\tilde Y}_j  \end{bmatrix}$, where $\mathbf{X}_i$ and $\mathbf{X}_j$ both have full column ranks. Meanwhile, let $\mathbf{W}_i = \mathbf{X}_i^\dagger \mathbf{Y}_i$, $\mathbf{\hat{W}}_j = \mathbf{X}_j^\dagger \mathbf{\bar Y}_j$ and $\mathbf{\check{W}}_j = \mathbf{X}_j^\dagger \mathbf{\tilde Y}_j$, we have
\begin{equation}
\label{eq:Theorem1_1}
  {\mathbf{W}}= \begin{bmatrix} \mathcal{W}_i\mathbf{W}_i + \mathcal{W}_j\mathbf{\hat W}_j & \mathcal{W}_j\mathbf{\check W}_j \end{bmatrix},
\end{equation}
where
\begin{equation}
\label{eq:Theorem1_2}
  \begin{cases}
\mathcal{W}_i = \mathbf{I} - \mathbf{M}_i^{-1} \mathbf{M}_j - \mathbf{M}_i^{-1} \mathbf{M}_j (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_j, \\
\mathcal{W}_j = \mathbf{I} - \mathbf{M}_j^{-1} \mathbf{M}_i - \mathbf{M}_j^{-1} \mathbf{M}_i (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_i, \\
\mathbf{M}_i = \mathbf{X}_i^\top \mathbf{X}_i, \quad \quad \mathbf{M}_j = \mathbf{X}_j^\top \mathbf{X}_j.
\end{cases}
\end{equation}


\noindent \textit{Proof.} Firstly, according to Lemma 1, it is established that:
\begin{equation}
\label{eq:appendix2_1}
  \mathbf{X}^{\dagger}=\begin{bmatrix}\bar{\mathbf{U}}&\bar{\mathbf{V}}\end{bmatrix},
\end{equation}
where
\begin{equation}
\label{eq:appendix2_2}
\begin{cases}
\mathbf{\bar{U}} = \left[\mathbf{I} - \mathbf{R}_i \mathbf{M}_j - \mathbf{R}_i \mathbf{M}_j (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_j \right] \mathbf{X}_i^\dagger \\
\mathbf{\bar{V}} = \left[\mathbf{I} - \mathbf{R}_j \mathbf{M}_i - \mathbf{R}_j \mathbf{M}_i (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_i \right] \mathbf{X}_j^\dagger
\end{cases},
\begin{cases}
\mathbf{M}_i = \mathbf{X}_i^\top \mathbf{X}_i \\
\mathbf{M}_j = \mathbf{X}_j^\top \mathbf{X}_j
\end{cases},
\begin{cases}
\mathbf{R}_i = \mathbf{M}_i^{-1} \\
\mathbf{R}_j = \mathbf{M}_j^{-1}
\end{cases}.
\end{equation}

\noindent Consequently, $\mathbf{W}$ can be computed as follows:
\begin{equation}
\label{eq:appendix2_3}
  \mathbf{W} = \mathbf{X}^{\dagger} \mathbf{Y} = \begin{bmatrix} \mathbf{\bar{U}} & \mathbf{\bar{V}} \end{bmatrix} \begin{bmatrix} \mathbf{Y}_i & \textbf{0} \\ \mathbf{\bar Y}_j & \mathbf{\tilde Y}_j  \end{bmatrix} = \begin{bmatrix} \mathbf{\bar{U}}\mathbf{Y}_i + \mathbf{\bar{V}}\mathbf{\bar Y}_j & \mathbf{\bar{V}} \mathbf{\tilde Y}_j \end{bmatrix}.
\end{equation}

\noindent By substituting (\ref{eq:appendix2_2}) into (\ref{eq:appendix2_3}), we obtain
\begin{equation}
\label{eq:appendix2_4}
\begin{aligned}
  \mathbf{W} =  \lbrack \left(\mathbf{I} - \mathbf{R}_i \mathbf{M}_j - \mathbf{R}_i \mathbf{M}_j (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_j \right) \mathbf{X}_i^\dagger \mathbf{Y}_i + \left(\mathbf{I}-\mathbf{R}_j\mathbf{M}_i-\mathbf{R}_j\mathbf{M}_i(\mathbf{M}_i+\mathbf{M}_j)^{-1}\mathbf{M}_i\right)\mathbf{X}_j^\dagger \mathbf{\bar Y}_j \\
  \left(\mathbf{I}-\mathbf{R}_j\mathbf{M}_i-\mathbf{R}_j\mathbf{M}_i(\mathbf{M}_i+\mathbf{M}_j)^{-1}\mathbf{M}_i\right)\mathbf{X}_j^\dagger \mathbf{\tilde Y}_j\rbrack.
\end{aligned}
\end{equation}

\noindent That is,
\begin{equation}
\label{eq:appendix2_5}
  \mathbf{W}= \begin{bmatrix} \mathcal{W}_i\mathbf{W}_i + \mathcal{W}_j\mathbf{\hat W}_j & \mathcal{W}_j\mathbf{\check W}_j \end{bmatrix},
\end{equation}
where
\begin{equation}
\label{eq:appendix2_6}
  \begin{cases}
\mathcal{W}_i = \mathbf{I} - \mathbf{R}_i \mathbf{M}_j - \mathbf{R}_i \mathbf{M}_j (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_j\\
\mathcal{W}_j = \mathbf{I} - \mathbf{R}_j \mathbf{M}_i - \mathbf{R}_j \mathbf{M}_i (\mathbf{M}_i + \mathbf{M}_j)^{-1} \mathbf{M}_i
\end{cases}
\begin{cases}
\mathbf{M}_i = \mathbf{X}_i^\top \mathbf{X}_i\\
\mathbf{M}_j = \mathbf{X}_j^\top \mathbf{X}_j
\end{cases}
\begin{cases}
\mathbf{R}_i = \mathbf{M}_i^{-1}\\
\mathbf{R}_j = \mathbf{M}_j^{-1}
\end{cases}.
\end{equation}

\hfill $\blacksquare$




\noindent \textbf{Theorem 1.} Let $\mathbf{X}_{1:k} = \begin{bmatrix} \mathbf{X}_{1:k-1} \\ \mathbf{X}_k\end{bmatrix}$ and $\mathbf{Y}_{1:k} = \begin{bmatrix} \mathbf{Y}_{1:k-1} & \textbf{0} \\ \mathbf{\bar Y}_{k} & \mathbf{\tilde Y}_{k}  \end{bmatrix}$ represent the feature matrix and label matrix of the first $k$ clients' complete dataset, where $\mathbf{X}_{1:k-1}$ and $\mathbf{X}_k$ both have full column ranks. Meanwhile, we denote $\mathbf{W}_{\mathrm{agg},k}$ as the optimal weights of the global model, i.e., $\mathbf{W}_{\mathrm{agg},k} = \mathbf{X}_{1:k}^\dagger \mathbf{Y}_{1:k}$, we have
\begin{equation}
\label{eq:Theorem1_1}
  {\mathbf{W}_{\mathrm{agg},k}}= \begin{bmatrix} \mathcal{W}_{\mathrm{agg},k-1} \mathbf{W}_{\mathrm{agg},k-1} + \mathcal{W}_k\mathbf{\hat W}_k & \mathcal{W}_k\mathbf{\check W}_k \end{bmatrix},
\end{equation}
where
\begin{equation}
\label{eq:Theorem1_2}
  \begin{cases}
\mathcal{W}_{\mathrm{agg},k} = \mathbf{I} - (\mathbf{M}_{\mathrm{agg}, k-1})^{-1} \mathbf{M}_k (\mathbf{I} + (\mathbf{M}_{\mathrm{agg}, k})^{-1} \mathbf{M}_k), \\
\mathcal{W}_k = \mathbf{I} - \mathbf{M}_k^{-1} \mathbf{M}_{\mathrm{agg}, k-1} (\mathbf{I} + \mathbf{M}_{\mathrm{agg}, k}^{-1} \mathbf{M}_{\mathrm{agg}, k-1}), \\
\mathbf{M}_{\mathrm{agg}, k} = \sum_i^k \mathbf{M}_i, \quad \mathbf{M}_i = \mathbf{X}_i^\top \mathbf{X}_i.
\end{cases}
\end{equation}

\noindent \textit{Proof.}
Building upon the \textbf{Proposition 3}, we can further extend the model aggregation from two clients to multiple clients.
when the $k$-th client connects to the server, the server's global model is denoted as $\mathbf{W}_{\mathrm{agg},k-1}$ and the client's local model as $\mathbf{\hat W}_k, \mathbf{\check W}_k$. 
Following aggregation, the global model $\mathbf{W}_{\mathrm{agg},k}$ can be computed as follows:

\begin{equation}
\label{eq:aggregation_1}
\mathbf{W}_{\mathrm{agg},k} = \begin{bmatrix} \mathbf{\mathcal{W}}_{\mathrm{agg},k}\mathbf{W}_{\mathrm{agg},k-1} + \mathcal{W}_k\mathbf{\hat W}_k & \mathcal{W}_k\mathbf{\check W}_k \end{bmatrix},
\end{equation}

\noindent By substituting $\mathbf{M}_{\mathrm{agg},k-1}$, $\mathbf{M}_{k}$ for $\mathbf{M}_u$, $\mathbf{M}_v$ in (\ref{eq:Theorem1_2}), we can obtain:
\begin{equation}
  \mathbf{M}_{\mathrm{agg},k} = \mathbf{M}_{\mathrm{agg},k-1} + \mathbf{M}_k = \sum_i^k \mathbf{M}_{k}.
\end{equation}


\noindent Hence,
% \begin{equation}
% \label{eq:aggregation_2}
%   \begin{cases}
% \mathcal{W}_{\mathrm{agg},k} = \mathbf{I} - (\mathbf{M}_{\mathrm{agg}, k-1})^{-1} \mathbf{M}_k (\mathbf{I} + (\mathbf{M}_{\mathrm{agg}, k})^{-1} \mathbf{M}_k), \\
% \mathcal{W}_k = \mathbf{I} - \mathbf{M}_k^{-1} \mathbf{M}_{\mathrm{agg}, k-1} (\mathbf{I} + \mathbf{M}_{\mathrm{agg}, k}^{-1} \mathbf{M}_{\mathrm{agg}, k-1}), \\
% \mathbf{M}_{\mathrm{agg}, k} = \sum_i^k \mathbf{M}_i, \quad \mathbf{M}_i = \mathbf{X}_i^\top \mathbf{X}_i.
% \end{cases}
% \end{equation}
\begin{equation}
\begin{aligned}
    \mathcal{W}_{\mathrm{agg},k} &= \mathbf{I} - (\mathbf{M}_{\mathrm{agg}, k-1})^{-1} \mathbf{M}_k (\mathbf{I} + (\mathbf{M}_{\mathrm{agg}, k-1} + \mathbf{M}_{k})^{-1} \mathbf{M}_k) \\
    &= \mathbf{I} - (\mathbf{M}_{\mathrm{agg}, k-1})^{-1} \mathbf{M}_k (\mathbf{I} + (\mathbf{M}_{\mathrm{agg}, k})^{-1} \mathbf{M}_k),
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
    \mathcal{W}_k &= \mathbf{I} - \mathbf{M}_k^{-1} \mathbf{M}_{\mathrm{agg}, k-1} (\mathbf{I} + (\mathbf{M}_{\mathrm{agg}, k-1} + \mathbf{M}_{k})^{-1} \mathbf{M}_{\mathrm{agg}, k-1}) \\
    &= \mathbf{I} - \mathbf{M}_k^{-1} \mathbf{M}_{\mathrm{agg}, k-1} (\mathbf{I} + \mathbf{M}_{\mathrm{agg}, k}^{-1} \mathbf{M}_{\mathrm{agg}, k-1}).
\end{aligned}
\end{equation}


\hfill $\blacksquare$











\noindent \textbf{Proposition 4.} Let $\mathbf{W}$ and $\mathbf{W}^\mathrm{r}$ represent the outcomes of \eqref{eq:Theorem1-1} and \eqref{eq:server-3} with the dataset $\mathbf{X} = \begin{bmatrix} \mathbf{X}_i \\ \mathbf{X}_j\end{bmatrix}$ and $\mathbf{Y} = \begin{bmatrix} \mathbf{Y}_i & \textbf{0} \\ \mathbf{\bar Y}_j & \mathbf{\tilde Y}_j  \end{bmatrix}$, their relationship can be established as follows:
\begin{equation}
\label{eq:Proposition4-1}
\mathbf{W}=(\mathbf{M}_i^{\mathrm{r}} + \mathbf{M}_j^{\mathrm{r}} - 2 \gamma \mathbf{I})^{-1} (\mathbf{M}_i^{\mathrm{r}} + \mathbf{M}_j^{\mathrm{r}}) \mathbf{W}^{\mathrm{r}},
\end{equation}
where
\begin{equation}
\label{eq:Proposition4-2}
  \mathbf{M}_i^\mathrm{r} = \mathbf{X}_i^\top \mathbf{X}_i + \gamma \mathbf{I}, \quad \mathbf{M}_j^\mathrm{r} = \mathbf{X}_j^\top \mathbf{X}_j + \gamma \mathbf{I}.
\end{equation}

\noindent \textit{Proof.} Initially, based on \eqref{eq:server-3}, we can obtain:
\begin{equation}
\mathbf{W}^\mathrm{r} = \begin{bmatrix} \mathbf{\mathcal{W}}_i^\mathrm{r}  \mathbf{W}_i^\mathrm{r} + \mathcal{W}_j^\mathrm{r}  \mathbf{\hat W}_j^\mathrm{r} & \mathcal{W}_j^\mathrm{r}  \mathbf{\check W}_j^\mathrm{r} \end{bmatrix},
\end{equation}
where
\begin{equation}
\begin{cases}
\mathcal{W}_i^\mathrm{r} = \mathbf{I} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{I} + (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_j),  \\
\mathcal{W}_j^\mathrm{r}  = \mathbf{I} - (\mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_i^\mathrm{r} (\mathbf{I} + (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_i^\mathrm{r}), \\
\mathbf{M}_i^\mathrm{r} = \mathbf{X}_i^\top \mathbf{X}_i +\gamma\mathbf{I}, \quad
\mathbf{M}_j^\mathrm{r} = \mathbf{X}_j^\top \mathbf{X}_j +\gamma\mathbf{I}.
\end{cases}
\end{equation}

\noindent Following this, given that $\mathbf{W}_i^\mathrm{r} = (\mathbf{X}_i^\top \mathbf{X}_i + \gamma \mathbf{I})^{-1} \mathbf{X}_i^\top \mathbf{Y}_i$ then
\begin{equation}
\label{eq:appendix3_3}
  \begin{aligned}
\mathcal{W}_{i}^{\mathrm{r}}\mathbf{{W}}_{i}^{\mathrm{r}} &= [\mathbf{I} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{I} + (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r})] (\mathbf{X}_i^\top \mathbf{X}_i + \gamma \mathbf{I})^{-1} \mathbf{X}_i^\top \mathbf{Y}_i \\
&= [\mathbf{I} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{I} + (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r})] (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{X}_i^\top \mathbf{Y}_i \\
&= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{I} + (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r})(\mathbf{M}_i^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i \\
&= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i .
% [\mathbf{I}-\mathbf{R}_i^\mathrm{r}\mathbf{M}_j^\mathrm{r}-\mathbf{R}_i^\mathrm{r}\mathbf{M}_j^\mathrm{r}(\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1}\mathbf{M}_j^\mathrm{r}]\mathbf{R}_i^\mathrm{r}\mathbf{X}_i^\top\mathbf{Y}_i\\
% &=[\mathbf{R}_i^\mathrm{r}-\mathbf{R}_i^\mathrm{r}\mathbf{M}_j^\mathrm{r}\mathbf{R}_i^\mathrm{r}-\mathbf{R}_i^\mathrm{r}\mathbf{M}_j^\mathrm{r}(\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1}\mathbf{M}_j^\mathrm{r}\mathbf{R}_i^\mathrm{r}]\mathbf{X}_i^\top\mathbf{Y}_i.
\end{aligned}
\end{equation}

\noindent Subsequently, based on the Woodbury Matrix Identity as presented in (\ref{eq:appendix1_9}), we substitute both $\mathbf{B}$ and $\mathbf{D}$ with $\mathbf{I}$. This adjustment allows us to derive:
\begin{equation}
\label{eq:appendix3_4}
(\mathbf{A}+\mathbf{E})^{-1}=\mathbf{A}^{-1}-\mathbf{A}^{-1}(\mathbf{A}^{-1}+\mathbf{E}^{-1})^{-1}\mathbf{A}^{-1}
\end{equation}

\noindent Further, it can be obtained:
\begin{equation}
\label{eq:appendix3_5}
\mathbf{A}^{-1}(\mathbf{A}^{-1}+\mathbf{E}^{-1})^{-1}\mathbf{A}^{-1} = \mathbf{A}^{-1} - (\mathbf{A}+\mathbf{E})^{-1}.
\end{equation}

\noindent Subsequently, replacing $\mathbf{A}^{-1}$ and $\mathbf{E}^{-1}$ in (\ref{eq:appendix3_5}) with $\mathbf{M}_i^\mathrm{r}$ and $\mathbf{M}_j^\mathrm{r}$ respectively, yields:
\begin{equation}
\label{eq:appendix3_6}
\mathbf{M}_j^\mathrm{r}(\mathbf{M}_j^\mathrm{r}+\mathbf{M}_i^\mathrm{r})^{-1}\mathbf{M}_j^\mathrm{r} = \mathbf{M}_j^\mathrm{r} - ( (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_j^\mathrm{r})^{-1} )^{-1}
\end{equation}

\noindent Similarly,
\begin{equation}
\label{eq:appendix3_7}
(\mathbf{M}_i^\mathrm{r})^{-1} ( (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_j^\mathrm{r})^{-1} )^{-1} (\mathbf{M}_i^\mathrm{r})^{-1} = (\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1}
\end{equation}

\noindent Initially, incorporating (\ref{eq:appendix3_6}) into (\ref{eq:appendix3_3}), we find:
\begin{equation}
\label{eq:appendix3_8}
\begin{aligned}
\mathbf{\mathcal{W}}_i^\mathrm{r}\mathbf{\hat{W}}_i^\mathrm{r} &= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r} + \mathbf{M}_j^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i \\
&= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_i^\mathrm{r})^{-1} \mathbf{M}_j^\mathrm{r} (\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} ( (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_j^\mathrm{r})^{-1} )^{-1} (\mathbf{M}_i^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i \\
&= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} ( (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_j^\mathrm{r})^{-1} )^{-1} (\mathbf{M}_i^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i
\end{aligned}
\end{equation}


\noindent Proceeding to integrate (\ref{eq:appendix3_5}) into (\ref{eq:appendix3_8}), we can determine:
\begin{equation}
\label{eq:appendix3_9}
\begin{aligned}
\mathbf{\mathcal{W}}_i^\mathrm{r} \mathbf{W}_i^\mathrm{r} 
&= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} ( (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_j^\mathrm{r})^{-1} )^{-1} (\mathbf{M}_i^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i \\
&= [(\mathbf{M}_i^\mathrm{r})^{-1} - (\mathbf{M}_i^\mathrm{r})^{-1} + (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1}] \mathbf{X}_i^\top \mathbf{Y}_i \\
&= (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1} \mathbf{X}_i^\top \mathbf{Y}_i.
\end{aligned}
\end{equation}

\noindent Similarly, we can obtain:
\begin{equation}
\label{eq:appendix3_10}
\mathbf{\mathcal{W}}_j^\mathrm{r} \mathbf{\hat{W}}_j^\mathrm{r} = (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1} \mathbf{X}_j^\top \mathbf{\bar Y}_j.
\end{equation}

\begin{equation}
\label{eq:appendix3_10}
\mathbf{\mathcal{W}}_j^\mathrm{r} \mathbf{\check{W}}_j^\mathrm{r} = (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1} \mathbf{X}_j^\top \mathbf{\tilde Y}_j.
\end{equation}

\noindent Combining (\ref{eq:appendix3_9}), (\ref{eq:appendix3_10}), and (\ref{eq:appendix3_1}) can be expressed as:
\begin{equation}
\label{eq:appendix3_11}
\begin{aligned}
\mathbf{W}^\mathrm{r} 
& = \begin{bmatrix} \mathbf{\mathcal{W}}_i^\mathrm{r}  \mathbf{W}_i^\mathrm{r} + \mathcal{W}_j^\mathrm{r}  \mathbf{\hat W}_j^\mathrm{r} & \mathcal{W}_j^\mathrm{r}  \mathbf{\check W}_j^\mathrm{r} \end{bmatrix}
 \\
& = (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r})^{-1} \begin{bmatrix} \mathbf{X}_i^\top \mathbf{Y}_i + \mathbf{X}_j^\top \mathbf{\bar Y}_j & \mathbf{X}_j^\top \mathbf{\tilde Y}_j\end{bmatrix}.
\end{aligned}
\end{equation}

\noindent Given that ${\mathbf{W}} = \mathbf{X}^\dagger \mathbf{Y}$, where $\mathbf{X} = \begin{bmatrix} \mathbf{X}_i \\ \mathbf{X}_j \end{bmatrix}$ and $\mathbf{Y} = \begin{bmatrix} \mathbf{Y}_i & \textbf{0} \\ \mathbf{\bar Y}_j & \mathbf{\tilde Y}_j \end{bmatrix}$, ${\mathbf{W}}$ can be calculated as:
\begin{equation}
\label{eq:appendix3_12}
\begin{aligned}
\mathbf{W}& =\mathbf{X}^\dagger\mathbf{Y}\\
&=(\mathbf{X}^\mathrm{T}\mathbf{X})^{-1}\mathbf{X}^\mathrm{T}\mathbf{Y} \\
&=(\begin{bmatrix}\mathbf{X}_i^\mathrm{T}&\mathbf{X}_j^\mathrm{T}\end{bmatrix}\begin{bmatrix}\mathbf{X}_i\\\mathbf{X}_j\end{bmatrix})^{-1}\begin{bmatrix}\mathbf{X}_i^\mathrm{T}&\mathbf{X}_j^\mathrm{T}\end{bmatrix}\begin{bmatrix} \mathbf{Y}_i & \textbf{0} \\ \mathbf{\bar Y}_j & \mathbf{\tilde Y}_j \end{bmatrix} \\
&=(\mathbf{X}_i^\top\mathbf{X}_i+\mathbf{X}_j^\top\mathbf{X}_j)^{-1}\begin{bmatrix} \mathbf{X}_i^\top\mathbf{Y}_i + \mathbf{X}_j^\top\mathbf{\bar Y}_j & \mathbf{X}_j^\top\mathbf{\tilde Y}_j\end{bmatrix} \\
&=(\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r} - 2 \gamma \mathbf{I})^{-1}\begin{bmatrix} \mathbf{X}_i^\top\mathbf{Y}_i + \mathbf{X}_j^\top\mathbf{\bar Y}_j & \mathbf{X}_j^\top\mathbf{\tilde Y}_j\end{bmatrix}.
\end{aligned}
\end{equation}


\noindent Observing (\ref{eq:appendix3_11}) and (\ref{eq:appendix3_12}) reveals the following relationship between:
\begin{equation}
\begin{aligned}
    &(\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r} - 2 \gamma \mathbf{I}) \mathbf{W} = (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r}) \mathbf{W}^\mathrm{r} \\
    \Rightarrow & \mathbf{W} = (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r} - 2 \gamma \mathbf{I})^{-1} (\mathbf{M}_i^\mathrm{r}+\mathbf{M}_j^\mathrm{r}) \mathbf{W}^\mathrm{r}.
\end{aligned}
\end{equation}

\hfill $\blacksquare$








\noindent \textbf{Theorem 2.} Let $\mathbf{W}_{\mathrm{agg},k}$ and $\mathbf{W}_{\mathrm{agg},k}^\mathrm{r}$ represent the outcomes of \eqref{eq:Theorem1-1} and \eqref{eq:server-3} with the dataset $\{ \mathbf{X}_{1:k} , \mathbf{Y}_{1:k} \}$, their relationship can be established as follows:
\begin{equation}
\label{eq:Theorem2_1}
    \mathbf{W}_{\mathrm{agg},k} = (\mathbf{M}_{\mathrm{agg},k}^{\mathrm{r}} - k\gamma \mathbf{I})^{-1} \mathbf{M}_{\mathrm{agg},k}^{\mathrm{r}} \mathbf{W}_{\mathrm{agg},k}^{\mathrm{r}},
\end{equation}
where
\begin{equation}
\label{eq:Theorem2_2}
  \mathbf{M}_{\mathrm{agg},k}^\mathrm{r} = \sum_{i=1}^k \mathbf{M}_i^\mathrm{r}, \quad \mathbf{M}_i^\mathrm{r} = \mathbf{X}_i^\top \mathbf{X}_i + \gamma \mathbf{I}.
\end{equation}


\noindent \textit{Proof.}
Building upon the \textbf{Proposition 4}, we can further extend the model aggregation from two clients to multiple clients.
Specifically, we employ $\mathbf{W}_{\mathrm{agg},k-1}^\mathrm{r}$, $\mathbf{W}_{\mathrm{agg},k-1}$, $\mathbf{M}_{\mathrm{agg},k-1}^{\mathrm{r}}$, and $\mathbf{M}_k^\mathrm{r}$ to substitute for $\mathbf{W}^\mathrm{r}$, $\mathbf{W}$, $\mathbf{M}_{i}^{\mathrm{r}}$, and $\mathbf{M}_j^\mathrm{r}$ in  (\ref{eq:Proposition4-1}) and (\ref{eq:Proposition4-2}), i.e.
\begin{equation}
\label{eq:Theorem2_1}
    \mathbf{W}_{\mathrm{agg},k} = (\mathbf{M}_{\mathrm{agg},k-1}^{\mathrm{r}} + \mathbf{M}_{k}^{\mathrm{r}} - k \gamma \mathbf{I})^{-1} (\mathbf{M}_{\mathrm{agg},k-1}^{\mathrm{r}} + \mathbf{M}_{k}^{\mathrm{r}}) \mathbf{W}_{\mathrm{agg},k}^{\mathrm{r}}.
\end{equation}

\noindent Since 
\begin{equation}
\label{eq:Theorem2_2}
  \mathbf{M}_{\mathrm{agg},k}^\mathrm{r} = \sum_{i=1}^k \mathbf{M}_i^\mathrm{r}, \quad \mathbf{M}_i^\mathrm{r} = \mathbf{X}_i^\top \mathbf{X}_i + \gamma \mathbf{I},
\end{equation}
we can obtain:
\begin{equation}
\label{eq:Theorem2_1}
\begin{aligned}
    \mathbf{W}_{\mathrm{agg},k} &= (\mathbf{M}_{\mathrm{agg},k-1}^{\mathrm{r}} + \mathbf{M}_{k}^{\mathrm{r}} - k \gamma \mathbf{I})^{-1} (\mathbf{M}_{\mathrm{agg},k-1}^{\mathrm{r}} + \mathbf{M}_{k}^{\mathrm{r}}) \mathbf{W}_{\mathrm{agg},k}^{\mathrm{r}} \\
    &=(\mathbf{M}_{\mathrm{agg},k}^{\mathrm{r}} - k\gamma \mathbf{I})^{-1} \mathbf{M}_{\mathrm{agg},k}^{\mathrm{r}} \mathbf{W}_{\mathrm{agg},k}^{\mathrm{r}}.
\end{aligned}
\end{equation}

\hfill $\blacksquare$



























